Constructing Exact Confidence Regions on Parameter Manifolds of Non-Linear Models

Using the mathematical framework of information geometry, we introduce a novel method which allows one to efficiently determine the exact shape of simultaneous confidence regions for non-linearly parametrised models. Furthermore, we show how pointwise confidence bands around the model predictions can be constructed from detailed knowledge of the exact confidence region with little additional computational effort. We exemplify our methods using inference problems in cosmology and epidemic modelling. An open source implementation of the developed schemes is publicly available via the InformationGeometry.jl package for the Julia programming language.

==> arXiv/referencing.tex <==




%%%%%%%%%%%%% Referencing %%%%%%%%%%%%%
\makeatletter
\@ifclassloaded{beamer}{}{\usepackage[unicode]{hyperref}}
\makeatother
\hypersetup{hidelinks,breaklinks,linktoc=all,colorlinks=true,allcolors=black}
\usepackage[noabbrev,capitalise]{cleveref}
\usepackage{xstring}

% Leave these colors black for now, change to other style by activating fancy.tex
\definecolor{figcol}{RGB}{0,0,0}
\definecolor{eqncol}{RGB}{0,0,0}
\definecolor{seccol}{RGB}{0,0,0}

% Application of color to the number tags of equation and align etc. environments.
\makeatletter
\renewcommand{\eqref}[1]{\textup{\eqreftagform@{\ref{#1}}}}
\let\eqreftagform@\tagform@
\def\tagform@#1{%
	\maketag@@@{\color{eqncol}(\ignorespaces#1\unskip\@@italiccorr)}%
}
\makeatother



% Allow cleverref to infer that the "equation" label should be used for labels inside IEEE environments
% https://tex.stackexchange.com/questions/250733/ieeetran-cls-and-cleveref-the-special-case-of-ieeeeqnarray
% Does not appear to be working???
\makeatletter
\patchcmd{\@IEEEyesnumber}
{\stepcounter}
{\refstepcounter}
{}{}
\patchcmd{\@@IEEEeqnarray}
{\stepcounter}
{\refstepcounter}
{}{}
\patchcmd{\@@IEEEeqnarraycr}
{\stepcounter{IEEEsubequation}}
{\refstepcounter{IEEEsubequation}}
{}{}
\patchcmd{\@@IEEEeqnarraycr}
{\stepcounter{IEEEsubequation}}
{\refstepcounter{IEEEsubequation}}
{}{}
\patchcmd{\@@IEEEeqnarraycr}
{\stepcounter{IEEEequation}}
{\refstepcounter{IEEEequation}}
{}{}
\patchcmd{\@@IEEEeqnarraycr}
{\stepcounter{IEEEequation}}
{\refstepcounter{IEEEequation}}
{}{}
\makeatother




% Still a problem for "fig 1 to 3, 5 and 7". Color Crefnames already?

\IfStrEq*{\languagename}{ngerman}{%
	\newcommand{\crefrangeconjunction}{ bis }
	\newcommand{\crefpairconjunction}{ und }
}{
	\newcommand{\crefrangeconjunction}{ to }
	\newcommand{\crefpairconjunction}{ and }
}

%%%%%%%% Section
\makeatletter
% Word
\IfStrEq*{\languagename}{ngerman}{%
	\crefname{section}{Kapitel}{Kapitel}
	\Crefname{section}{Kapitel}{Kapitel}
}{
	\crefname{section}{section}{sections}
	\Crefname{section}{Section}{Sections}
}
% Basic
\crefformat{section}{#2\textcolor{seccol}{\cref@section@name~#1}#3}
\Crefformat{section}{#2\textcolor{seccol}{\Cref@section@name~#1}#3}
% Connected Range
\crefrangeformat{section}{\textcolor{seccol}{\cref@section@name@plural}~#3\textcolor{seccol}{#1}#4\crefrangeconjunction#5\textcolor{seccol}{#2}#6}
\Crefrangeformat{section}{\textcolor{seccol}{\Cref@section@name@plural}~#3\textcolor{seccol}{#1}#4\crefrangeconjunction#5\textcolor{seccol}{#2}#6}
% Non-connected Range
\crefmultiformat{section}{\textcolor{seccol}{\cref@section@name@plural}~#2\textcolor{seccol}{#1}#3}{\crefpairconjunction#2\textcolor{seccol}{#1}#3}{, #2\textcolor{seccol}{#1}#3}{\crefpairconjunction#2\textcolor{seccol}{#1}#3}
\Crefmultiformat{section}{\textcolor{seccol}{\Cref@section@name@plural}~#2\textcolor{seccol}{#1}#3}{\crefpairconjunction#2\textcolor{seccol}{#1}#3}{, #2\textcolor{seccol}{#1}#3}{\crefpairconjunction#2\textcolor{seccol}{#1}#3}
\makeatother


%%%%%%%% Figure
\makeatletter
% Word
\IfStrEq*{\languagename}{ngerman}{%
	\crefname{figure}{Abbildung}{Abbildungen}
	\Crefname{figure}{Abbildung}{Abbildungen}
}{
	\crefname{figure}{figure}{figures}
	\Crefname{figure}{Figure}{Figures}
}
% Basic
\crefformat{figure}{#2\textcolor{figcol}{\cref@figure@name~#1}#3}
\Crefformat{figure}{#2\textcolor{figcol}{\Cref@figure@name~#1}#3}
% Connected Range
\crefrangeformat{figure}{\textcolor{figcol}{\cref@figure@name@plural}~#3\textcolor{figcol}{#1}#4\crefrangeconjunction#5\textcolor{figcol}{#2}#6}
\Crefrangeformat{figure}{\textcolor{figcol}{\Cref@figure@name@plural}~#3\textcolor{figcol}{#1}#4\crefrangeconjunction#5\textcolor{figcol}{#2}#6}
% Non-connected Range
\crefmultiformat{figure}{\textcolor{figcol}{\cref@figure@name@plural}~#2\textcolor{figcol}{#1}#3}{\crefpairconjunction#2\textcolor{figcol}{#1}#3}{, #2\textcolor{figcol}{#1}#3}{\crefpairconjunction#2\textcolor{figcol}{#1}#3}
\Crefmultiformat{figure}{\textcolor{figcol}{\Cref@figure@name@plural}~#2\textcolor{figcol}{#1}#3}{\crefpairconjunction#2\textcolor{figcol}{#1}#3}{, #2\textcolor{figcol}{#1}#3}{\crefpairconjunction#2\textcolor{figcol}{#1}#3}
\makeatother


%%%%%%%% Table
\makeatletter
% Word
\IfStrEq*{\languagename}{ngerman}{%
	\crefname{table}{Tabelle}{Tabellen}
	\Crefname{table}{Tabelle}{Tabellen}
}{
	\crefname{table}{table}{tables}
	\Crefname{table}{Table}{Tables}
}
% Basic
\crefformat{table}{#2\textcolor{figcol}{\cref@table@name~#1}#3}
\Crefformat{table}{#2\textcolor{figcol}{\Cref@table@name~#1}#3}
% Connected Range
\crefrangeformat{table}{\textcolor{figcol}{\cref@table@name@plural}~#3\textcolor{figcol}{#1}#4\crefrangeconjunction#5\textcolor{figcol}{#2}#6}
\Crefrangeformat{table}{\textcolor{figcol}{\Cref@table@name@plural}~#3\textcolor{figcol}{#1}#4\crefrangeconjunction#5\textcolor{figcol}{#2}#6}
% Non-connected Range
\crefmultiformat{table}{\textcolor{figcol}{\cref@table@name@plural}~#2\textcolor{figcol}{#1}#3}{\crefpairconjunction#2\textcolor{figcol}{#1}#3}{, #2\textcolor{figcol}{#1}#3}{\crefpairconjunction#2\textcolor{figcol}{#1}#3}
\Crefmultiformat{table}{\textcolor{figcol}{\Cref@table@name@plural}~#2\textcolor{figcol}{#1}#3}{\crefpairconjunction#2\textcolor{figcol}{#1}#3}{, #2\textcolor{figcol}{#1}#3}{\crefpairconjunction#2\textcolor{figcol}{#1}#3}
\makeatother


%%%%%%%% Equation
\makeatletter
% Word
\IfStrEq*{\languagename}{ngerman}{%
	\crefname{equation}{Gleichung}{Gleichungen}
	\Crefname{equation}{Gleichung}{Gleichungen}
}{
	\crefname{equation}{equation}{equations}
	\Crefname{equation}{Equation}{Equations}
}
% Basic
\crefformat{equation}{#2\textcolor{eqncol}{\cref@equation@name~(#1)}#3}
\Crefformat{equation}{#2\textcolor{eqncol}{\Cref@equation@name~(#1)}#3}
% Connected Range
\crefrangeformat{equation}{\textcolor{eqncol}{\cref@equation@name@plural}~#3\textcolor{eqncol}{(#1)}#4\crefrangeconjunction#5\textcolor{eqncol}{(#2)}#6}
\Crefrangeformat{equation}{\textcolor{eqncol}{\Cref@equation@name@plural}~#3\textcolor{eqncol}{(#1)}#4\crefrangeconjunction#5\textcolor{eqncol}{(#2)}#6}
% Non-connected Range
\crefmultiformat{equation}{\textcolor{eqncol}{\cref@equation@name@plural}~#2\textcolor{eqncol}{(#1)}#3}{\crefpairconjunction#2\textcolor{eqncol}{(#1)}#3}{, #2\textcolor{eqncol}{(#1)}#3}{\crefpairconjunction#2\textcolor{eqncol}{(#1)}#3}
\Crefmultiformat{equation}{\textcolor{eqncol}{\Cref@equation@name@plural}~#2\textcolor{eqncol}{(#1)}#3}{\crefpairconjunction#2\textcolor{eqncol}{(#1)}#3}{, #2\textcolor{eqncol}{(#1)}#3}{\crefpairconjunction#2\textcolor{eqncol}{(#1)}#3}
\makeatother


%%%%%%% Algorithm, when defined
\makeatletter
% Word
\IfStrEq*{\languagename}{ngerman}{%
	\crefname{algorithm}{Algorithmus}{Algorithmen}
	\Crefname{algorithm}{Algorithmus}{Algorithmen}
}{
	\crefname{algorithm}{algorithm}{algorithms}
	\Crefname{algorithm}{Algorithm}{Algorithms}
}
% Basic
\crefformat{algorithm}{#2\textcolor{figcol}{\cref@algorithm@name~#1}#3}
\Crefformat{algorithm}{#2\textcolor{figcol}{\Cref@algorithm@name~#1}#3}
% Connected Range
\crefrangeformat{algorithm}{\textcolor{figcol}{\cref@algorithm@name@plural}~#3\textcolor{figcol}{#1}#4\crefrangeconjunction#5\textcolor{figcol}{#2}#6}
\Crefrangeformat{algorithm}{\textcolor{figcol}{\Cref@algorithm@name@plural}~#3\textcolor{figcol}{#1}#4\crefrangeconjunction#5\textcolor{figcol}{#2}#6}
% Non-connected Range
\crefmultiformat{algorithm}{\textcolor{figcol}{\cref@algorithm@name@plural}~#2\textcolor{figcol}{#1}#3}{\crefpairconjunction#2\textcolor{figcol}{#1}#3}{, #2\textcolor{figcol}{#1}#3}{\crefpairconjunction#2\textcolor{figcol}{#1}#3}
\Crefmultiformat{algorithm}{\textcolor{figcol}{\Cref@algorithm@name@plural}~#2\textcolor{figcol}{#1}#3}{\crefpairconjunction#2\textcolor{figcol}{#1}#3}{, #2\textcolor{figcol}{#1}#3}{\crefpairconjunction#2\textcolor{figcol}{#1}#3}
\makeatother



\NewDocumentCommand{\eqnref}{ o m }{\hyperref[#1]{\textcolor{eqncol}{#2}}}
\NewDocumentCommand{\figref}{ o m }{\hyperref[#1]{\textcolor{figcol}{#2}}}
\NewDocumentCommand{\secref}{ o m }{\hyperref[#1]{\textcolor{seccol}{#2}}}

%%%%%%%%%%%%% Referencing %%%%%%%%%%%%%




% Specify colors to be used for figures, equations and Citations to be used
\definecolor{seccol}{RGB}{50,50,50}
\definecolor{figcol}{RGB}{30,50,100}
\definecolor{eqncol}{RGB}{85,0,0}
\definecolor{refcol}{RGB}{1,50,32}
\definecolor{footnotecol}{RGB}{179,98,0}

\hypersetup{citecolor=refcol}



% Force IEEE to print equation numbers in color: eqncol
\def\theequationdis{\textcolor{eqncol}{(\theequation)}}% (1)
\def\theIEEEsubequationdis{\textcolor{eqncol}{(\theIEEEsubequation)}}% (1a)

% distance between lines in eqn arrays. Original: 3pt
\setlength{\jot}{5pt}
\setlength{\IEEEnormaljot}{5pt}

% Color Citations and their brackets
\makeatletter
\@ifpackageloaded{natbib}{\hypersetup{citecolor=refcol}
	\AtBeginDocument{\bibpunct{\textcolor{refcol}{[}}{\textcolor{refcol}{]}}{,}{n}{}{;}}}{}
% For superscript citations, replace n by s:
% \AtBeginDocument{\bibpunct{\textcolor{refcol}{[}}{\textcolor{refcol}{]}}{,}{s}{}{;}}}{}
\makeatother


% Colors of Footnotes
\renewcommand{\thefootnote}{\textcolor{footnotecol}{(\arabic{footnote})}}


\makeatletter
\@ifclassloaded{beamer}{}{\@ifpackageloaded{caption}{\captionsetup{labelfont={bf,color=figcol}}}{}}
\makeatother
